An Efficient Adversarial Attack for Tree Ensembles

We study the problem of efficient adversarial attacks on tree based ensembles such as gradient boosting decision trees (GBDTs) and random forests (RFs). Since these models are non-continuous step functions and gradient does not exist, most existing efficient adversarial attacks are not applicable. Although decision-based black-box attacks can be applied, they cannot utilize the special structure of trees. In our work, we transform the attack problem into a discrete search problem specially designed for tree ensembles, where the goal is to find a valid "leaf tuple" that leads to mis-classification while having the shortest distance to the original input. With this formulation, we show that a simple yet effective greedy algorithm can be applied to iteratively optimize the adversarial example by moving the leaf tuple to its neighborhood within hamming distance 1. Experimental results on several large GBDT and RF models with up to hundreds of trees demonstrate that our method can be thousands of times faster than the previous mixed-integer linear programming (MILP) based approach, while also providing smaller (better) adversarial examples than decision-based black-box attacks on general $\ell_p$ ($p=1, 2, \infty$) norm perturbations. Our code is available at https://github.com/chong-z/tree-ensemble-attack.

==> tables/attack-webspam.tex <==
\ratetable{0}{%
    title={Standard GBDT (webspam)},
    xlabel={\# of initial adversarial examples},
    ylabel={$\ell_{\infty}$ ratio},
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2
    },
    xmin=1, xmax=40,
    xtick={1, 10, 20, 30, 40},
    ymin=0.9, ymax=40,
    ytick={1, 2, 4, 8, 16, 32},
    width=0.4\textwidth,
    legend pos=south west,
    ymode=log,
    log ticks with fixed point,
    log basis y={2},
}{%MILP
    (1,1)(20,1)(40,1)
}{%Ours
    (1, 25.00)(3, 11.25)(4, 10.00)(5, 7.50)(6, 6.25)(7, 6.25)(8, 6.25)(9, 6.25)(10, 5.00)(15, 3.75)(20, 3.75)(30, 3.75)(40, 2.50)(50, 2.50)(60, 2.50)
}{%HSJA
    (1,28.75)(20,28.75)(40,28.75)
}{%SignOPT
    (1,16.25)(20,16.25)(40,16.25)
}{1}

\ratetable{0}{%
    title={Robust GBDT (webspam)},
    xlabel={\# of initial adversarial examples},
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2
    },
    xmin=1, xmax=40,
    xtick={1, 10, 20, 30, 40},
    ymin=0.9, ymax=10,
    width=0.4\textwidth,
    ymode=log,
    log ticks with fixed point,
    log basis y={2},
}{%MILP
    (1,1)(20,1)(40,1)
}{%Ours
    (1, 4.00)(3, 2.93)(4, 2.57)(5, 2.43)(6, 2.29)(7, 2.21)(8, 2.21)(9, 2.14)(10, 2.14)(15, 2.07)(20, 1.93)(30, 1.79)(40, 1.71)(50, 1.71)(60, 1.64)
}{%HSJA
    (1,3.21)(20,3.21)(40,3.21)
}{%SignOPT
    (1,3.29)(20,3.29)(40,3.29)
}{1}





==> tables/notations.tex <==
\resizebox{.75\columnwidth}{!}{
\begin{tabular}{ccc}
\toprule
Notation & Definition \\ \midrule
% $\mathcal{T}$     & target ensemble with $K$ decision trees \\ 
$S^{(t)}$         & set of leaf nodes of tree $t$ \\
% $m^{(t)}(x)$      & mapping from input $x$ to the leaf node of tree $t$ \\
$\C(x)$           & $(i^{(1)}, \dots, i^{(K)})$, tuple of prediction leaves \\
$\CC$             & $\{\C(x) \mid \forall x \in \RR^d\}$, set of valid tuples \\
$B^i = (l_1^i, r_1^i] \times \dots \times (l_d^i, r_d^i]$             & bounding box of node $i$ \\
$B(\C(x)) = (l_1, r_1] \times \dots \times (l_d, r_d]$ & $\bigcap_{i \in \C(x)} B^i$, bounding box of input $x$ \\
\bottomrule
\end{tabular}
}

==> tables/robust.tex <==
\createtable{Robust GBDT}{$\ell_\infty$ Perturbation}{
MNIST 2 vs. 6 & .583 & 2.73s & .460 & 1.27s & .671 & .172s & .335 & 2.44s & .331 & .302s & .317 & 98.7s & 1.04 & 326.8X \\
breast-cancer & .421 & .351s & .421 & .071s & .419 & .0008s & .865 & .229s & .415 & .001s & .415 & .008s & 1.00 & 8.X \\
covtype & .065 & .465s & .101 & .210s & .097 & 3.28s & .055 & .968s & .047 & .053s & .044 & 518s* & 1.07 & 9773.6X \\
diabetes & .132 & .284s & .132 & .064s & .150 & .001s & .238 & .235s & .122 & .002s & .121 & .036s & 1.01 & 18.X \\
Fashion-MNIST & .269 & 4.33s & .158 & 1.94s & .602 & 6.15s & .104 & 5.95s & .098 & .403s & .078 & 29min* & 1.26 & 4367.2X \\
HIGGS & .015 & .403s & .016 & .152s & .053 & 57.2s* & .012 & .819s & .01 & .054s & .009 & 45min* & 1.11 & 50648.1X \\
ijcnn & .047 & .299s & .046 & .102s & .067 & .019s & .041 & .334s & .038 & .006s & .036 & 3.60s & 1.06 & 600.X \\
MNIST & .536 & 4.24s & .399 & 1.73s & .690 & 4.89s & .308 & 4.96s & .298 & .315s & .278 & 13min* & 1.07 & 2469.8X \\
webspam & .046 & .785s & .045 & .446s & .060 & .659s & .019 & .867s & .016 & .038s & .014 & 51.2s & 1.14 & 1347.4X \\
}

\smallskip

\createtable{Robust GBDT}{$\ell_2$ Perturbation}{
MNIST 2 vs. 6 & 2.85 & 6.79s & 3.10 & 1.53s & 2.95 & .172s & 1.30 & 3.61s & .968 & .401s & .803 & 17.3s & 1.21 & 43.1X \\ 
breast-cancer & .465 & .559s & .501 & .072s & .456 & .0008s & .954 & .245s & .452 & .001s & .452 & .007s & 1.00 & 7.X \\ 
covtype & .077 & .957s & .167 & .221s & .141 & 3.29s & .096 & 1.05s & .063 & .054s & .059 & 280s & 1.07 & 5185.2X \\ 
diabetes & .154 & .538s & .182 & .060s & .177 & .0009s & .295 & .288s & .144 & .002s & .143 & .024s & 1.01 & 12.X \\ 
Fashion-MNIST & 1.83 & 10.3s & 1.46 & 2.10s & 3.79 & 6.15s & .517 & 10.2s & .326 & .468s & .251 & 99.3s & 1.30 & 212.2X \\ 
HIGGS & .021 & .867s & .022 & .152s & .093 & 56.6s* & .023 & .871s & .016 & .054s & .015 & 15min* & 1.07 & 17148.1X \\ 
ijcnn & .054 & .513s & .057 & .099s & .094 & .019s & .071 & .364s & .048 & .007s & .046 & .728s & 1.04 & 104.X \\ 
MNIST & 3.75 & 9.47s & 3.34 & 1.93s & 4.15 & 4.89s & 1.42 & 8.67s & .996 & .395s & .701 & 200s & 1.42 & 506.3X \\ 
webspam & .091 & 3.19s & .116 & .528s & .145 & .652s & .066 & 1.02s & .039 & .036s & .033 & 12.0s & 1.18 & 333.3X \\ 
}

